Incident-Specific Cyber Insurance

In the current market practice, many cyber insurance products offer a coverage bundle for losses arising from various types of incidents, such as data breaches and ransomware attacks, and the coverage for each incident type comes with a separate limit and deductible. Although this gives prospective cyber insurance buyers more flexibility in customizing the coverage and better manages the risk exposures of sellers, it complicates the decision-making process in determining the optimal amount of risks to retain and transfer for both parties. This paper aims to build an economic foundation for these incident-specific cyber insurance products with a focus on how incident-specific indemnities should be designed for achieving Pareto optimality for both the insurance seller and buyer. Real data on cyber incidents is used to illustrate the feasibility of this approach. Several implementation improvement methods for practicality are also discussed.

==> parts/intro.tex <==
\section{Introduction}
In May 2021, Colonial Pipeline, one of the largest oil pipeline systems in the United States (US), was hit by a ransomware attack and had a shutdown for five days; see \citet{OfficeCybersecurity2021}. In November 2020, Amazon Web Services, a major cloud service provider that many businesses rely on, had a severe outage triggered by an operating system configuration; see \citet{Greene2020}. In 2017, Equifax, one of the three largest US credit reporting agencies, experienced a major data breach that exposed the private records of nearly 150 million American citizens; see \citet{Equifax2017}. In 2016, a class action was brought against Meta Platforms (formerly known as Facebook) for failing to comply with the Biometric Information Privacy Act in Illinois, and the case was settled for \$650 million in 2021; see \citet{Holland2021}. These examples illustrate the extraordinary exposure of modern businesses to cyber risk and their possible devastating consequences. 

The events listed above represent a wide range of incidents that are considered cyber-related, and they are common in this digital world where business operations rely heavily on data and cyber systems. To mitigate the aftermath impact of such incidents, cyber insurance products are designed for businesses to purchase. The insurability of cyber losses is examined in \citet{dacorogna_building_2023}, in which their loss expectations are shown to be finite. These cyber insurance products typically cover losses resulting from various perils. As summarized in \citet{Romanosky2019, Marotta2017, Woods2017}, some cyber insurance policies indemnify losses caused by ransomware, and some policies cover liabilities resulting from data breaches. It is also not unusual for a single policy to cover multiple types of cyber incidents. In this paper, our focus is on those policies that offer coverage for multiple perils, which are referred to as \textit{incident-specific cyber insurance}.

\subsection*{Need for incident-specific cyber insurance}
Incident-specific cyber insurance products are in line with businesses' needs for cyber risk management. 

A definition of cyber risk commonly adopted in practice and literature is ``cyber risks are operational risks to information and technology assets that have consequences affecting the confidentiality, availability, and integrity of information and information systems''; see \citet{Cebula2010}. Aligning to this idea, the National Institute of Standards and Technology (NIST) Cybersecurity Framework, from which many cybersecurity standards for critical infrastructure sectors are derived, considers data security from the perspectives of data confidentiality, integrity, and availability and proposes a comprehensive set of best practices; see \citet{NIST2018}. In \citet{Eling2019}, the authors argued that cyber risks are subcategories of operational risk and used cyber-related data from a database of operational losses to model the loss of four types of cyber incidents, including the ones caused by actions of people, system failure, internal process failure, and external events. In \citet{Amin2017}, the author considered the same four categories of cyber risks and used Bayesian networks to model the relationship between risk categories and risk factors. In \citet{Ghadge2019}, the authors proposed a different set of incident types for supply chain cyber risk management, including physical threats, breakdown, indirect attacks, direct attacks, and insider threats. 

Provided that cyber risk is a collective term referring to the risks of multiple types of cyber incidents, and businesses typically demand a risk management strategy that is holistic and, at the same time, can address the subtle differences among various incident types, purchasing an incident-specific cyber insurance policy is then a natural choice for businesses to meet such a need.

\subsection*{Existing incident-specific cyber insurance}
To ensure risk exposures are manageable, many incident-specific cyber insurance policies come with sublimits and separate deductibles for individual coverages. For example, \citet{AIG2019} allows for setting limits and deductibles individually for events such as cyber extortion and computer crime. \citet{Romanosky2019} surveyed 67 policies and found many of them use sublimits. In this paper, these sublimits and deductibles shall be referred to as \textit{incident-specific limits}, or simply \textit{limits}, and \textit{incident-specific deductibles} or \textit{deductibles}. The scope of this study though does not include the cases in which there is a limit or deductible at the aggregate policy level, which shall be deferred to future research.

Although insurers can shield them from excessive exposures using those risk-sharing provisions, such policy designs complicate the process of shopping for cyber insurance coverage for prospective buyers. Given that most companies have difficulties in determining the appropriate amount of coverage (see \citet{johansmeyer_cybersecurity_2021}), this problem will only be more of an obstacle that hinders cyber insurance purchases if companies have to impromptu configure the amounts of coverage for individual incident types.  

\subsection*{Proposed workflow for determining coverage}
Provided that incident-specific cyber insurance is a norm in practice but lacks a technical foundation that justifies the determination of coverage amounts,
it is in the interests of both insurers and companies, who seek insurance coverage, to make the process of determining incident-specific coverage easy to understand, compatible with the existing underwriting procedures, and mutually beneficial to both parties. To this end, we shall address the aforementioned problem of determining incident-specific coverage from a bilateral perspective. 

Drawing inspiration from \citet{Asimit2021}, which shows that an environment-specific indemnity profile could be Pareto optimal for both the buyer and seller, in this paper, we propose an economically sound workflow that determines the appropriate amount of incident-specific coverage. By doing so, it helps the insured and the insurer reach a Pareto optimality, such that the risk taken by either of the two parties cannot be further reduced without increasing the other's risk. How such a problem should be formulated and how both parties' risks are measured are elaborated in Section \ref{sec:formulation}.

The diagram in Figure \ref{fig:workflow_diagram} illustrates this workflow, which consists of three major parts: (I) the \textit{incident-specific cyber insurance problem}, which serves as the central pillar of this workflow and assigns optimal amounts of risk to the policyholder and the insurer; (II) \textit{model inputs}, in which severity and incident type can be estimated and statistically learned based on historical cyber incident data and the underwriting process, together with the policyholder's and insurer's preferences information for the decision-making part; and (III) the \textit{solver} for the optimal insurance problem, which can be implemented using either an exact method or an approximated but quick method depending on whether there is a time constraint. The solver produces specifications of the incident-specific insurance coverage, which is the final and desired outcome of this workflow.
%Each of these three parts shall be elaborated in this paper. 
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{manuscript_figs/incident-specific-diagram.pdf}
    \caption{Workflow of designing incident-specific cyber insurance coverage}
    \label{fig:workflow_diagram}
\end{figure}

Regarding Part (III), a practical scenario is that the insurer needs to provide a quote and a coverage to a prospective customer on-the-fly. We shall show that using the exact method may result in a long waiting time, and thus the quick method, which generates the results almost instantly, can be a workaround in that situation.

In this paper, we shall detail the key components of the proposed workflow for designing incident-specific cyber insurance coverage, and then demonstrate it with numerical examples.


\subsection*{Findings and contributions}
First, based on the incident-specific insurance design problem, the cyber insurance contract supplied by the proposed workflow must be reducing the aggregate cyber risk of a company, as an insurance buyer, and the insurer after the risk transfer; the contract must also be mutually beneficial to both the insured and the insurer since a paid premium is less than the buyer's cyber risk reduction while is able to cover the risk taken by the insurer. However, their aggregate cyber risk reduction is not necessarily effective, in the sense that some insurance buyers might pay more premium than their reduction in the aggregate risk with the insurer; this is indeed observed from the numerical examples presented in Section \ref{sec:fun_approx}. 
% from the numerical examples, for some cyber insurance buyers, their paid premium would always be more than the reduction in the aggregate risk.
%First, while, based on the incident-specific insurance design problem, a company, as an insurance buyer, experiences a risk reduction greater than a paid premium which is able to cover the taken risk by the insurer, for some companies, an appropriate amount of premium for the incident-specific insurance contract supplied by the proposed workflow could be less than the reduction of aggregate risk taken by both parties after the risk transfer. This illustrates the effectiveness of the incident-specific cyber insurance described in this paper in reducing cyber risk and being mutually beneficial to both the insured and the insurer.
% {\color{red}One is that when a company, as an insurance buyer, pays an appropriate amount of premium for an incident-specific insurance contract supplied by the proposed workflow, the company will experience a risk reduction greater than the paid premium. On the other hand, although the insurer has an increased risk for covering the insured's losses, the collected premium exceeds the taken risk. Consequentially, the aggregate risk taken by both parties is reduced. }
Second, the proposed workflow is computationally tractable in scenarios that require the specifications of an incident-specific policy to be delivered promptly, such as quick quote and coverage services, comparing to other conventional methods.

Therefore, the contributions of this paper are as follows. Firstly, cyber insurance policies commonly cover multiple perils, but the determination of incident-specific coverage amounts lacks justification in practice and literature. The proposed workflow leads to insurance specifications that are justified and economically sound to both the insured and the insurer. Secondly, the proposed workflow is data-driven and compatible with the existing underwriting procedures. All the data required by this workflow can be obtained from public or proprietary sources by underwriters, which results in no additional work on the frontend. Thirdly, we show that, from the numerical examples, while the designed incident-specific cyber insurance contract must be mutually beneficial to the insured and the insurer, their aggregate cyber risk reduction might not be always effective. 
%{\color{red}We also showed using real data that an incident-specific cyber policy as an outcome of the proposed workflow makes both the insured and the insurer better off; \textit{i.e.}, the insured enjoys a reduced risk greater than the paid premium, and the insurer collects more premium than the risk taken.}
Lastly, this paper overcomes the possible computational challenges arising from the implementation of such a workflow, making it versatile and adaptable to different scenarios depending on the amount of time permitted to produce results. 

The rest of this paper is organized as follows. Section \ref{sec:formulation} formulates the problem of designing incident-specific cyber insurance as an optimization problem. Section \ref{sec:model_inputs} discusses the method and the data that we used to obtain the necessary model inputs. Given the model inputs, Section \ref{sec:cme} describes the Cross Entropy Method and how it is used to solve the proposed problem as well as presents and discusses some numerical results. Section \ref{sec:fun_approx} presents the use of function approximation to address some computational challenges in the process of solving the optimization problem. We conclude in the last section with discussions of potential applications and future works.

% A survey conducted by PartnerRe (2018) shows that one of the major complaints that policyholders have about cyber insurance is the insufficient coverage. The insufficiency is two-fold. One is that many cyber insurance policies have a limited scope of coverage in terms of the covered loss types. The other is that there is a capacity constraint in the market, which may prevent policyholders from getting enough coverage from a single insurer. 

==> parts/intro_old.tex <==
\section{Introduction}
\subsection*{Broad definition of cyber risks}
In May 2021, Colonial Pipeline, one of the largest oil pipeline systems in the United States (US), was hit by a ransomware attack and had a shutdown for five days; see \citet{OfficeCybersecurity2021}. In November 2020, Amazon Web Services, a major cloud service provider that many businesses rely on, had a severe outage triggered by an operating system configuration; see \citet{Greene2020}. In 2017, Equifax, one of the three largest US credit reporting agencies, experienced a major data breach that exposed the private records of nearly 150 million American citizens; see \citet{Equifax2017}. In 2016, a class action was brought against Meta Platforms (formerly known as Facebook) for failing to comply with the Biometric Information Privacy Act in Illinois, and the case was settled for \$650 million in 2021; see \citet{Holland2021}. These examples illustrate the extraordinary exposure of modern businesses to cyber risk and the possible devastating consequences of cyber risk. 

In this paper, we adhere to the definition of cyber risk given in \citet{Cebula2010} that cyber risks are ``operational risks to information and technology assets that have consequences affecting the confidentiality, availability, and integrity of information and information systems''. This definition of cyber risk is broad, and the events listed above represent historical incidents of distinct characteristics that are considered cyber risks. This definition is also adopted in other research works centered around the assessment and management of cyber risks. In \citet{Eling2019}, the authors argued that cyber risks are subcategories of operational risk and used cyber-related data from a database of operational losses to model the loss of four types of cyber incidents, including the ones caused by actions of people, system failure, internal process failure, and external events. In \citet{Amin2017}, the author considered the same four categories of cyber risks and used Bayesian networks to model the relationship between risk categories and risk factors. In \citet{Ghadge2019}, the authors proposed a different set of incident types for supply chain cyber risk management, including physical threats, breakdown, indirect attacks, direct attacks, and insider threats. 

% In this paper, these listed events represent different historical incidents that are considered cyber-related risks, as we adhere to the definition given in \citet{Cebula2010} that cyber risks are ``operational risks to information and technology assets that have consequences affecting the confidentiality, availability, and integrity of information and information systems''. This definition is also often adopted in other research works centered around the assessment and management of cyber risks. In \citet{Eling2019}, the authors argued that cyber risks are subcategories of operational risk and used cyber-related data from a database of operational losses to model the loss of four types of cyber incidents, including the ones caused by actions of people, system failure, internal process failure, and external events. In \citet{Amin2017}, the author considered the same four categories of cyber risks and used Bayesian networks to model the relationship between risk categories and risk factors. In \citet{Ghadge2019}, the authors proposed a different set of incident types for supply chain cyber risk management, including physical threats, breakdown, indirect attacks, direct attacks, and insider threats. 

The National Institute of Standards and Technology (NIST) Cybersecurity Framework, from which many cybersecurity standards for critical infrastructure sectors are derived, also considers data security from the perspectives of data confidentiality, integrity, and availability. It suggests mitigation strategies for a list of possible adverse scenarios that may affect data-at-rest, data-in-transit, and other information assets (see \citet{NIST2018}). 

The research work and the NIST framework presented above, which represent the academic and risk management practices perspectives, respectively, suggest that cyber risks generally cannot be regarded as a whole. Instead, a wide range of incident types should be considered and treated separately. As it seems intuitive that cyber risks have such diversity, it is worthwhile to emphasize this property of cyber risks, which naturally leads to the discussion on a comprehensive yet incident-specific solution to cyber risk management, whereof the comprehensiveness and incident-specificity mean that the risks of a set of cyber incidents can be addressed simultaneously and differently.

\subsection*{Insurance coverage for specific cyber incident types}

Cyber insurance can be used by businesses to partially transfer their cyber risks to a third party, \textit{i.e.}, the insurer. The broad meaning of cyber risks coincides with the convention that many insurance products, which are designated for a variety of loss events, are often indifferently referred to as cyber insurance. As summarized in \citet{Romanosky2019, Marotta2017, Woods2017}, some cyber insurance policies reimburse losses caused by ransomware, and some policies cover liabilities resulting from data breaches. It is also not unusual for a single policy to cover multiple types of cyber incidents.

To ensure risk exposures are manageable, many cyber insurance policies come with sublimits and separate retentions for individual coverages. For example, \citet{AIG2019} allows for setting limits and retentions individually for events such as cyber extortion and computer crime. \citet{Romanosky2019} surveyed 67 policies and found many of them use sublimits. In this paper, these sublimits and retentions shall be referred to as \textit{incident-specific limits}, or simply \textit{limits}, and \textit{incident-specific retentions} or \textit{retentions}. The scope of this study though does not include the cases, in which there is a limit or retention at the aggregate policy level.

Those incident-specific limits and retentions complicate the process of shopping for cyber insurance coverage and bring up a critical question for cyber insurance buyers: How much of each type of cyber risk should be retained, and how much of it should be transferred to an insurer? For insurers, the question is: How much of each type of cyber risk should be accepted? In this paper, we shall address these questions from a bilateral perspective.
By determining the appropriate amount of incident-specific indemnities, the insured and the insurer will reach a Pareto optimality, such that the risk taken by either of the two parties cannot be further reduced without increasing the other's risk. How such a problem should be formulated and how both parties' risks are measured are elaborated in Section \ref{sec:formulation}.
% By determining the appropriate amount of incident-specific indemnities, the insured and the insurer can agree that both objectives are improved the most, and neither of the two cannot be improved further without compromising the other. 

 

% Since the rapid adoption of the Internet in the 90s, the breakthrough of smartphones in the 00s, and the most recent advancement in cryptocurrency and artificial intelligence in the 10s, human beings have been becoming increasingly more reliant on the information technology and showing no sign of turning back. Among all, modern corporations have been benefiting most from these technological advancements. Businesses extensively rely on technologies, such as automation and information systems, to gradually improve their operation efficiencies, and hence expansions.

% However, the history consistently shows us the flip side of the coin. The 2014 JPMorgan Chase data breach, 2017 WannaCry ransomware attack, 2017 Equifax data breach, and the most recent leak of information on login credentials of workers at the World Health Organization in 2020, are only the tip of the iceberg in the history of major cyber incidents. While the business world takes substantial benefits in this cyber era, such as cost efficiency, productivity improvement, and communication advancement, people should always bear in mind the cyber risk associated with such a technological dependence due to any potential internal and external disturbance. Indeed, cyber risk has been ranked as one of the top three, if not the foremost, emerging risks in recent years.

% In acknowledgement of the rise of cyber risk, cyber insurance is one of the most crucial risk mitigation strategies. The cyber insurance market has been expanding in the United States, with 2.25 billion dollars of premium being written in 2019. %https://www.insurancejournal.com/news/national/2020/07/22/576507.html
%Similar to any traditional property and casualty insurance, cyber loss coverage enables the insured corporate to swiftly recover from cyber losses by sharing risk with an insurer. In the current market practice, most of the cyber insurance policies solely provide coverages for particular types of cyber incidents. If a cyber incident falls within the types specified in the contract, indemnities will be issued with deductibles and limits, which are the same among various covered incidents; on the other hand, if that incident lies outside the specified types, no indemnity will be provided to the insured. The most common types of cyber incidents being indemnifiable are data breach and privacy violation.%Linfeng please double check


% Similar to any traditional property and casualty insurance, cyber loss coverage enables the insured corporate to swiftly recover from cyber losses by sharing risk with an insurer. In the current market practice, most of the cyber insurance policies solely provide coverage for particular types of cyber losses. If a cyber loss falls within the types that are specified in the contract, indemnities will be issued with deductibles and limits; on the other hand, if that loss lies outside the specified types, no indemnity will be provided to the insured. The most common types of cyber losses being indemnifiable include losses associated with data breach events, such as data-recreation costs and notification costs, and losses caused by privacy violations, such as legal defense costs and liabilities.


% While it seems reasonable in practice to provide coverage only for some cyber incident types, such an ad-hoc exclusion lacks a scientific foundation. A business corporation, as a customer, would simply lose faith in these cyber policies' providers. Moreover, the market convention of designing same deductibles and limits among multiple covered incidents is impromptu, which undermines the potential discrepancy of cyber loss distributions among incident types. An insurance company offering these coverages would easily provide excessive under-insurance or over-insurance for some cyber incident types. These would potentially impose challenges to both cyber insurance buyers and sellers for further market growth in the future.

It has been shown in \citet{Asimit2021} that an environment-specific indemnity profile could be Pareto optimal for both the buyer and seller. In our context, this means the insurance buyer and the insurance company could reach a consensus that the cyber insurance coverage with incident-specific retentions and limits is mutually beneficial to both parties in the sense that neither of the two can further lower its own risk without increasing the risk borne by the other party. In order to determine the Pareto optimal incident-specific cyber insurance coverage and to ensure the policies do not degenerate back to any traditional coverage, \textit{i.e.}, non-incident-specific coverage, a thorough cyber risk assessment is demanded, particularly on (i) the conditional probability of each cyber incident type given an array of company's and cyber incident's characteristics, and (ii) the conditional cyber loss distribution due to each cyber incident type. Those risk assessment results will then lead to the design of optimal cyber insurance contracts that provides incident-specific coverage. 


\subsection*{Optimal incident-specific cyber insurance}
Provided that incident-specific cyber insurance is a norm in practice but lacks a scientific foundation, in this paper, we propose an actuarially sound workflow for insurers to design optimal incident-specific insurance contracts. The diagram in Figure \ref{fig:workflow_diagram} illustrates this workflow, which consists of three major parts: (1) the \textit{incident-specific cyber insurance problem}, which serves as the central piece of this workflow and assigns optimal amounts of risk to the policyholder and the insurer; (2) \textit{model inputs}, which can be estimated or predicted based on historical cyber incident data and the underwriting process; and (3) the \textit{solver} for the optimal insurance problem, which can be implemented using either an exact method or an approximated but quick method depending on whether there is a time constraint. The solver produces specifications of the optimal incident-specific insurance, which is the final and desired outcome of this workflow. 

Regarding Part (3), a practical scenario is that the insurer needs to provide a quote to a prospective customer on the fly. We shall show that using the exact method may result in a long waiting time, and thus the quick method, which generates the results instantly, can be a workaround in that situation. Each of the three parts is elaborated on in this paper. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{manuscript_figs/incident-specific-diagram.pdf}
    \caption{Workflow of designing optimal incident-specific cyber insurance}
    \label{fig:workflow_diagram}
\end{figure}

% TODO: contributions can be improved
The contribution of this paper is four-fold. First, this paper is data-evident in the sense that, instead of theoretically deriving the optimality of incident-specific cyber insurance coverage as in \citet{Asimit2021}, we make use of the actual cyber incident dataset acquired from Advisen Ltd., which is a leading insurance data provider, to conduct our analysis. Second, since part (ii) of the cyber risk assessment demands statistical distribution fitting and testing, various statistical learning models are explored in this paper to address part (i) of the cyber risk assessment. Third, since incident-specific cyber insurance provides coverage for some, if not all, cyber incident types, this paper provides a data-driven justification for such an incident-specific cyber insurance contract to ensure that such an emerging insurance market is sustainable and growing. Lastly, based on the theoretical work of \citet{Asimit2021}, this paper demonstrates how the optimal design of incident-specific cyber insurance can be implemented for practical use and how some computational challenges can be overcome by our approach.   

The rest of this paper is organized as follows. Section \ref{sec:formulation} formulates the problem of designing an incident-specific cyber insurance as an optimization problem. Section \ref{sec:model_inputs} discusses the method and the data that we used to obtain the necessary model inputs. Given the model inputs, Section \ref{sec:cme} describes the Cross Entropy Method and how it is used to solve the proposed problem, and presents some numerical results. Section \ref{sec:fun_approx} discusses the use of function approximation to address some computational challenges in the process of solving the optimization problem. We conclude in the last section with discussions of potential applications and future works.

% A survey conducted by PartnerRe (2018) shows that one of the major complaints that policyholders have about cyber insurance is the insufficient coverage. The insufficiency is two-fold. One is that many cyber insurance policies have a limited scope of coverage in terms of the covered loss types. The other is that there is a capacity constraint in the market, which may prevent policyholders from getting enough coverage from a single insurer. 
